How to Search the Internet Archive Without Indexing It

Significant parts of cultural heritage are produced on the web during the last decades. While easy accessibility to the current web is a good baseline, optimal access to the past web faces several challenges. This includes dealing with large-scale web archive collections and lacking of usage logs that contain implicit human feedback most relevant for today's web search. In this paper, we propose an entity-oriented search system to support retrieval and analytics on the Internet Archive. We use Bing to retrieve a ranked list of results from the current web. In addition, we link retrieved results to the WayBack Machine; thus allowing keyword search on the Internet Archive without processing and indexing its raw archived content. Our search system complements existing web archive search tools through a user-friendly interface, which comes close to the functionalities of modern web search engines (e.g., keyword search, query auto-completion and related query suggestion), and provides a great benefit of taking user feedback on the current web into account also for web archive search. Through extensive experiments, we conduct quantitative and qualitative analyses in order to provide insights that enable further research on and practical applications of web archives.

==> archivelinking.tex <==





==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we proposed a web archive search prototype that for the
first time supports entity-oriented queries on the Internet
Archive. Our system leverages Bing and the WayBack Machine to allow
users to search the past web. We provided search functionalities
including keyword search, query auto-completion, query suggestion, and
a ranked list of results, which are close to the current search engine
systems. We conducted extensive analyses that shed light on web
archive search. In addition, we included a longer discussion of future
work as well as insights on the ideas/challenges for the next steps
for our web archive search investigations.

